U-Flow: A U-shaped Normalizing Flow for Anomaly Detection with Unsupervised Threshold

In this work we propose a one-class self-supervised method for anomaly segmentation in images that benefits both from a modern machine learning approach and a more classic statistical detection theory. The method consists of four phases. First, features are extracted using a multi-scale image Transformer architecture. Then, these features are fed into a U-shaped Normalizing Flow (NF) that lays the theoretical foundations for the subsequent phases. The third phase computes a pixel-level anomaly map from the NF embedding, and the last phase performs a segmentation based on the a contrario framework. This multiple hypothesis testing strategy permits the derivation of robust unsupervised detection thresholds, which are crucial in real-world applications where an operational point is needed. The segmentation results are evaluated using the Mean Intersection over Union (mIoU) metric, and for assessing the generated anomaly maps we report the area under the Receiver Operating Characteristic curve (AUROC), as well as the Area Under the Per-Region-Overlap curve (AUPRO). Extensive experimentation in various datasets shows that the proposed approach produces state-of-the-art results for all metrics and all datasets, ranking first in most MVTec-AD categories, with a mean pixel-level AUROC of 98.74%. Code and trained models are available at https:// github.com/mtailanian/uflow.

==> tables/_more_results.tex <==
\renewcommand{\b}[1]{\textbf{#1}}
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcommand{\vtext}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}

\begin{table*}[t]

  \small
  \centering
    
  \begin{tabularx}{1\textwidth}{ @{\hskip 8pt} c @{\hskip 8pt} | @{\hskip 10pt} l @{\hskip 8pt} YYYY Y Y}
    \toprule
    \multicolumn{1}{c}{} & & \textbf{LGG~MRI} & \textbf{STC} & \textbf{BT01} & \textbf{BT02} & \textbf{BT03} & \textbf{BT~AV.}\\
    \midrule
        
    \multirow{4}{*}{\vtext{\rotatebox[origin=c]{90}{\textbf{AUROC}}}}
        & \textbf{FastFlow}          & 82.51     & 95.51     & 95.98     & 96.69     & 99.32     & 97.33     \\
        & \textbf{CFlow}             & 86.41     & \b{96.90} & 94.29     & 96.13     & 99.58     & 96.67     \\
        & \textbf{CS-Flow}           &  81.82    & 86.68     & 91.66     & 94.89     & 99.10     & 95.22     \\
        & \textbf{U-Flow (ours)}     & \b{93.55} & 87.19     & \b{97.70} & \b{96.93} & \b{99.76} & \b{98.13} \\
    \midrule
    \multirow{4}{*}{\vtext{\rotatebox[origin=c]{90}{\textbf{AUPRO}}}}
        & \textbf{FastFlow}          & 47.48     & 73.67      & 76.23     & 62.39     & 96.60     & 78.41     \\
        & \textbf{CFlow}             & 59.47     & \b{82.05}  & 60.19     & 54.72     & 98.32     & 71.08     \\
        & \textbf{CS-Flow}           & 37.30     & 54.04      & 73.75     & 47.18     & 94.45     & 71.79     \\
        & \textbf{U-Flow (ours)}     & \b{71.74} & 47.54      & \b{80.06} & \b{66.49} & \b{98.83} & \b{81.79} \\
    \midrule
    % \multirow{4}{*}{\vtext{\rotatebox[origin=c]{90}{\textbf{IMAGE}}}} & 
    %     \textbf{FastFlow}            & 61.49     & 74.04      & \b{100.0} & \b{89.13} & 96.65     & 95.26     \\
    %     & \textbf{CFlow}             & 42.56     & 66.39      & 94.95     & 79.68     & \b{99.96} & 91.53     \\
    %     & \textbf{CS-Flow}           & 67.41     & \b{98.46}  & 99.81     & 87.26     & 99.94     & 95.67     \\
    %     & \textbf{U-Flow (ours)}     & \b{72.60} & 64.59      & 99.42     & 88.72     & 99.72     & \b{95.95} \\
    % \midrule
    \multirow{7}{*}{\vtext{\rotatebox[origin=c]{90}{\textbf{IoU}}}} 
        & \textbf{FastFlow (Fair)}   & 0.010     & 0.235     & 0.366     & 0.479     & 0.583     & 0.476     \\
        & \textbf{FastFlow (Oracle)} & 0.217     & \b{0.737} & 0.446     & \b{0.481} & 0.751     & 0.559     \\
        & \textbf{CFlow (Fair)}      & 0.209     & 0.462     & 0.458     & 0.414     & 0.774     & 0.549     \\
        & \textbf{CFlow (Oracle)}    & 0.218     & 0.462     & 0.464     & 0.448     & 0.924     & 0.612     \\
        & \textbf{CS-Flow (Fair)}    & 0.206     & 0.421     & 0.352     & 0.135     & 0.874     & 0.454     \\
        & \textbf{CS-Flow (Oracle)}  & 0.218     & 0.489     & 0.378     & 0.234     & 0.929     & 0.514     \\    
        & \textbf{U-Flow (ours)}     & \b{0.219} & 0.462     & \b{0.488} & 0.288     & \b{0.936} & \b{0.571} \\
        
    \bottomrule
  \end{tabularx}
  \caption{Results for LGG MRI~\cite{buda2019association-lggmri}, ShanghaiTech Campus (STC)~\cite{liu2018ano_pred-stc}, and BeanTeach (BT)~\cite{mishra2021vt-beantech} datasets. Comparison with best-performing flow-based models: FastFlow~\cite{yu2021fastflow}, CFlow~\cite{gudovskiy2022cflow}, and CS-Flow~\cite{csflow-rudolph2022fully}. For almost all metrics and datasets, our method obtains the best results, outperforming the other methods. %``Image" metric refers to image-level \textit{AUROC}, and for 
  Both \textit{AUROC} and \textit{AUPRO} refer to the pixel-level metric (localization task). dFor IoU, both the ``Fair'' and ``Oracle''-like thresholds are presented for all competitors.}
  \label{tab:more_results}
\end{table*}

==> tables/_table_iou.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table}[t]

  \small

  \centering
  \begin{tabularx}{1\columnwidth}{@{}c@{\hskip 5pt} | YYY @{\hskip 10pt}| YYYY}
  % \begin{tabular}{@{}c@{\hskip 5pt}|c@{\hskip 5pt}c@{\hskip 5pt}c|c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}}
\toprule
& \multicolumn{3}{c|}{\textbf{Oracle threshold}} & \multicolumn{4}{c}{\textbf{Fair threshold}} \\
\cmidrule{2-8} 
% \textbf{Cat}
\begin{tabular}{@{}c@{}}\textbf{Cate-}\\ \textbf{gory}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Fast}\\ \textbf{Flow}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{C-} \\ \textbf{Flow} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Ours} \\ \textbf{NFA} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Fast} \\ \textbf{Flow} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{C-} \\ \textbf{Flow} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Ours} \\ \textbf{AS} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Ours} \\ \textbf{NFA} \end{tabular} \\
\midrule
\textbf{Carpet}      & 0.474          & 0.380          & \textbf{0.571} & 0.315          & 0.333          & 0.234          & \textbf{0.566} \\
\textbf{Grid}        & \textbf{0.300} & 0.263          & 0.249          & 0.274          & 0.125          & \textbf{0.358} & 0.226          \\
\textbf{Leather}     & 0.388          & 0.391          & \textbf{0.415} & 0.349          & 0.344          & 0.042          & \textbf{0.391} \\
\textbf{Tile}        & 0.553          & 0.392          & \textbf{0.611} & 0.418          & 0.286          & \textbf{0.617} & 0.600          \\
\textbf{Wood}        & 0.412          & 0.432          & \textbf{0.478} & 0.279          & 0.250          & 0.193          & \textbf{0.467} \\
\midrule
\textbf{Av. Texture} & 0.425          & 0.379          & \textbf{0.465} & 0.327          & 0.268          & 0.289          & \textbf{0.450} \\
\midrule
\textbf{Bottle}      & 0.667          & \textbf{0.735} & 0.623          & 0.494          & \textbf{0.737} & 0.233          & 0.623          \\
\textbf{Cable}       & 0.375          & 0.230          & \textbf{0.553} & 0.375          & 0.185          & 0.285          & \textbf{0.553} \\
\textbf{Capsule}     & \textbf{0.276} & 0.235          & 0.228          & \textbf{0.242} & 0.219          & 0.108          & 0.228          \\
\textbf{HazleNut}    & \textbf{0.559} & 0.539          & 0.541          & \textbf{0.558} & 0.244          & 0.279          & 0.539          \\
\textbf{MetalNut}    & 0.457          & 0.390          & \textbf{0.584} & 0.428          & 0.325          & 0.417          & \textbf{0.584} \\
\textbf{Pill}        & \textbf{0.501} & 0.370          & 0.433          & \textbf{0.471} & 0.338          & 0.245          & 0.428          \\
\textbf{Screw}       & 0.347          & 0.229          & \textbf{0.363} & 0.315          & 0.201          & 0.134          & \textbf{0.344} \\
\textbf{Toothbrush}  & 0.438          & 0.387          & \textbf{0.637} & 0.326          & 0.381          & 0.411          & \textbf{0.633} \\
\textbf{Transistor}  & 0.470          & 0.429          & \textbf{0.721} & 0.071          & 0.147          & 0.074          & \textbf{0.721} \\
\textbf{Zipper}      & 0.488          & 0.376          & \textbf{0.498} & 0.315          & 0.150          & 0.285          & \textbf{0.481} \\
\midrule
\textbf{Av. Object}  & 0.459          & 0.392          & \textbf{0.518} & 0.360          & 0.293          & 0.247          & \textbf{0.514} \\
\midrule
\midrule
\textbf{Total}       & 0.448          & 0.388          & \textbf{0.501} & 0.349          & 0.284          & 0.261          & \textbf{0.492} \\
\bottomrule
  \end{tabularx}
  \caption{Segmentation IoU comparison with the best performing methods in the literature: FastFlow~\cite{yu2021fastflow} and CFlow~\cite{gudovskiy2022cflow}, for the oracle-like and fair thresholds defined in Section~\ref{sec:segmentation-results}. Our method largely outperforms all others, even comparing the proposed automatic threshold with their oracle-like threshold.}
  \label{tab:iou}
  % \vspace{-10pt}
\end{table}


==> tables/_table_iou_new.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[t]

  \small

  \centering
  \begin{tabularx}{1\textwidth}{c | YYYY | YYYYY}
  % \begin{tabular}{@{}c@{\hskip 5pt}|c@{\hskip 5pt}c@{\hskip 5pt}c|c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}}
\toprule
& \multicolumn{4}{c|}{\textbf{Oracle threshold}} & \multicolumn{5}{c}{\textbf{Fair threshold}} \\
\cmidrule{2-10} 
% \textbf{Cat}
\begin{tabular}{@{}c@{}}\textbf{Cate-}\\ \textbf{gory}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Fast}\\ \textbf{Flow}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{C-} \\ \textbf{Flow} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{CS-} \\ \textbf{Flow} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Ours} \\ \textbf{NFA} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Fast} \\ \textbf{Flow} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{C-} \\ \textbf{Flow} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{CS-} \\ \textbf{Flow} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Ours} \\ \textbf{AS} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Ours} \\ \textbf{NFA} \end{tabular} \\
\midrule
\textbf{Carpet}      & 0.474          & 0.380          & 0.351          & \textbf{0.571} & 0.315          & 0.333          & 0.341          & 0.234          & \textbf{0.566} \\
\textbf{Grid}        & 0.300          & 0.263          & \textbf{0.348} & 0.249          & 0.274          & 0.125          & 0.348          & \textbf{0.358} & 0.226          \\
\textbf{Leather}     & 0.388          & 0.391          &  0.298         & \textbf{0.415} & 0.349          & 0.344          & 0.282          & 0.042          & \textbf{0.391} \\
\textbf{Tile}        & 0.553          & 0.392          &  0.491         & \textbf{0.611} & 0.418          & 0.286          & 0.254          & \textbf{0.617} & 0.600          \\
\textbf{Wood}        & 0.412          & 0.432          &  0.339         & \textbf{0.478} & 0.279          & 0.250          & 0.067          & 0.193          & \textbf{0.467} \\
\midrule
\textbf{Av. Texture} & 0.425          & 0.379          & 0.365          & \textbf{0.465} & 0.327          & 0.268          & 0.258          & 0.289          & \textbf{0.450} \\
\midrule
\textbf{Bottle}      & 0.667          & \textbf{0.735} & 0.410          & 0.623          & 0.494          & \textbf{0.737} & 0.393          & 0.233          & 0.623          \\
\textbf{Cable}       & 0.375          & 0.230          & 0.501          & \textbf{0.553} & 0.375          & 0.185          & 0.366          & 0.285          & \textbf{0.553} \\
\textbf{Capsule}     & \textbf{0.276} & 0.235          & 0.274          & 0.228          & 0.242          & 0.219          & \textbf{0.267} & 0.108          & 0.228          \\
\textbf{HazleNut}    & \textbf{0.559} & 0.539          & 0.465          & 0.541          & \textbf{0.558} & 0.244          & 0.274          & 0.279          & 0.539          \\
\textbf{MetalNut}    & 0.457          & 0.390          & 0.463          & \textbf{0.584} & 0.428          & 0.325          & 0.408          & 0.417          & \textbf{0.584} \\
\textbf{Pill}        & \textbf{0.501} & 0.370          & 0.232          & 0.433          & \textbf{0.471} & 0.338          & 0.226          & 0.245          & 0.428          \\
\textbf{Screw}       & 0.347          & 0.229          & 0.311          & \textbf{0.363} & 0.315          & 0.201          & 0.304          & 0.134          & \textbf{0.344} \\
\textbf{Toothbrush}  & 0.438          & 0.387          & 0.314          & \textbf{0.637} & 0.326          & 0.381          & 0.300          & 0.411          & \textbf{0.633} \\
\textbf{Transistor}  & 0.470          & 0.429          & 0.659          & \textbf{0.721} & 0.071          & 0.147          & 0.641          & 0.074          & \textbf{0.721} \\
\textbf{Zipper}      & 0.488          & 0.376          & 0.408          & \textbf{0.498} & 0.315          & 0.150          & 0.408          & 0.285          & \textbf{0.481} \\
\midrule
\textbf{Av. Object}  & 0.459          & 0.392          & 0.404          & \textbf{0.518} & 0.360          & 0.293          & 0.359          & 0.247          & \textbf{0.514} \\
\midrule
\midrule
\textbf{Total}       & 0.448          & 0.388          & 0.391          & \textbf{0.501} & 0.349          & 0.284          & 0.325          & 0.261          & \textbf{0.492} \\
\bottomrule
  \end{tabularx}
  \caption{Segmentation IoU comparison with the best flow-based methods in the literature: FastFlow~\cite{yu2021fastflow}, CFlow~\cite{gudovskiy2022cflow}, and CS-Flow~\cite{csflow-rudolph2022fully}, for the oracle-like and fair thresholds defined in Section~\ref{sec:segmentation-results}. Our method largely outperforms all others, even comparing the proposed automatic threshold with their oracle-like threshold.}
  \label{tab:iou}
  % \vspace{-10pt}
\end{table*}


==> tables/table_miou.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

% \newcommand\bb[1]{\underline{\textbf{#1}}}
\newcommand\bb[1]{\textbf{#1}}

\begin{table*}[t]

  \small

  \centering
  \begin{tabularx}{1\textwidth}{c | YYYY | YYYY}
  % \begin{tabular}{@{}c@{\hskip 5pt}|c@{\hskip 5pt}c@{\hskip 5pt}c|c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}}
\toprule
& \multicolumn{4}{c|}{\textbf{Oracle threshold}} & \multicolumn{4}{c}{\textbf{Fair threshold}} \\
\cmidrule{2-9} 
% \textbf{Cat}
\textbf{Category}& \begin{tabular}{@{}c@{}}\textbf{Fast}\\ \textbf{Flow}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{C-} \\ \textbf{Flow} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{CS-} \\ \textbf{Flow} \end{tabular} & \textbf{Ours} & \begin{tabular}{@{}c@{}}\textbf{Fast} \\ \textbf{Flow} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{C-} \\ \textbf{Flow} \end{tabular} & \begin{tabular}{@{}c@{}}\textbf{CS-} \\ \textbf{Flow} \end{tabular} & \textbf{Ours} \\
\midrule
\textbf{Carpet}      & 0.5451      & 0.4519 & 0.3521 & \bb{0.5642} & 0.4267      & 0.2393      & 0.3420 & \bb{0.5144} \\
\textbf{Grid}        & \bb{0.4664} & 0.4077 & 0.3498 & 0.4314      & 0.2235      & 0.3413      & 0.3488 & \bb{0.4307} \\
\textbf{Leather}     & \bb{0.5483} & 0.4818 & 0.2986 & 0.3966      & \bb{0.5241} & 0.3096      & 0.2823 & 0.3772      \\
\textbf{Tile}        & 0.5564      & 0.3705 & 0.4906 & \bb{0.6216} & 0.4342      & 0.3105      & 0.2544 & \bb{0.6187} \\
\textbf{Wood}        & 0.4792      & 0.3767 & 0.3400 & \bb{0.5517} & 0.4584      & 0.2433      & 0.0806 & \bb{0.5427} \\
\midrule
\textbf{Av. Texture} & \bb{0.5191} & 0.4177 & 0.3662 & 0.5131      & 0.4134      & 0.2888      & 0.2616 & \bb{0.4967} \\
\midrule
\textbf{Bottle}      & 0.5750      & 0.6503 & 0.4098 & \bb{0.6175} & 0.4053      & \bb{0.6434} & 0.3935 & 0.5754      \\
\textbf{Cable}       & 0.5375      & 0.4009 & 0.5018 & \bb{0.6508} & 0.4807      & 0.2299      & 0.3668 & \bb{0.6491} \\
\textbf{Capsule}     & 0.3439      & 0.3040 & 0.2739 & \bb{0.3868} & 0.3160      & 0.3002      & 0.2669 & \bb{0.3796} \\
\textbf{HazleNut}    & 0.4723      & 0.5610 & 0.4654 & \bb{0.6515} & 0.4671      & 0.4831      & 0.2747 & \bb{0.6478} \\
\textbf{MetalNut}    & 0.5801      & 0.3981 & 0.4631 & \bb{0.6091} & 0.5801      & 0.2998      & 0.4165 & \bb{0.6064} \\
\textbf{Pill}        & 0.4616      & 0.3121 & 0.2324 & \bb{0.4804} & 0.4051      & 0.3096      & 0.2260 & \bb{0.4803} \\
\textbf{Screw}       & 0.2562      & 0.3039 & 0.3137 & \bb{0.3801} & 0.2375      & 0.2755      & 0.3049 & \bb{0.3726} \\
\textbf{Toothbrush}  & 0.3625      & 0.3347 & 0.3160 & \bb{0.4187} & 0.3007      & 0.2416      & 0.3016 & \bb{0.4121} \\
\textbf{Transistor}  & 0.6337      & 0.6000 & 0.6622 & \bb{0.7349} & 0.0597      & 0.2981      & 0.6516 & \bb{0.7106} \\
\textbf{Zipper}      & \bb{0.5772} & 0.5001 & 0.4092 & 0.5427      & 0.4184      & 0.2403      & 0.4082 & \bb{0.5391} \\
\midrule
\textbf{Av. Object}  & 0.4800      & 0.4365 & 0.4048 & \bb{0.5473} & 0.3671      & 0.3322      & 0.3611 & \bb{0.5373} \\
\midrule
\midrule
\textbf{Total}       & 0.4930      & 0.4302 & 0.3919 & \bb{0.5359} & 0.3825      & 0.3177      & 0.3279 & \bb{0.5238} \\
\bottomrule
  \end{tabularx}
  \caption{Segmentation \textit{mIoU} comparison for MVTec-AD, with the best flow-based methods in the literature: FastFlow~\cite{yu2021fastflow}, CFlow~\cite{gudovskiy2022cflow}, and CS-Flow~\cite{csflow-rudolph2022fully}, for the oracle-like and fair thresholds defined in Section~\ref{sec:segmentation-results}. Our method largely outperforms all others, and even exhibits a better performance comparing the proposed automatic threshold with their oracle-like threshold.}
  \label{tab:miou}
  % \vspace{-10pt}
\end{table*}

